Test Time Transform Prediction for Open Set Histopathological Image Recognition

Tissue typology annotation in Whole Slide histological images is a complex and tedious, yet necessary task for the development of computational pathology models. We propose to address this problem by applying Open Set Recognition techniques to the task of jointly classifying tissue that belongs to a set of annotated classes, e.g. clinically relevant tissue categories, while rejecting in test time Open Set samples, i.e. images that belong to categories not present in the training set. To this end, we introduce a new approach for Open Set histopathological image recognition based on training a model to accurately identify image categories and simultaneously predict which data augmentation transform has been applied. In test time, we measure model confidence in predicting this transform, which we expect to be lower for images in the Open Set. We carry out comprehensive experiments in the context of colorectal cancer assessment from histological images, which provide evidence on the strengths of our approach to automatically identify samples from unknown categories. Code is released at https://github.com/agaldran/t3po .

==> 4_discussion.tex <==
\section{Conclusion}
Imbalanced data is present in almost any medical image analysis task. 
Therefore, designing techniques for learning in such regimes is a challenge of great clinical significance. 
This paper introduces Balanced-MixUp to deal with heavy imbalanced data distributions by means of the combination of the popular MixUp regularization technique and modified training data sampling strategies. 
Balanced-MixUp is easy to implement and delivers consistent performance improvements when compared with other popular techniques. Its extension to other tasks beyond image classification represents a promising future research direction. 








==> abstract <==
Highly imbalanced datasets are ubiquitous in medical image  classification problems. In such problems, it is often the case that rare classes associated to less prevalent diseases are severaly under represented in labeled databases, typically resulting in poor performance of machine learning algorithms due to overfitting in the learning process. In this paper, we propose a novel mechanism for sampling training data based on the popular MixUp regularization technique, which we refer to as Balanced-MixUp. In short, Balanced-MixUp simultaneously performs regular (\textit{i.e.}, instance-based) and balanced (\textit{i.e.}, class-based) sampling of the training data. The resulting two sets of samples are then mixed-up to create a more balanced training distribution from which a neural network can effectively learn without incurring in heavily under-fitting the minority classes. We experiment with a highly imbalanced dataset of retinal images (55K samples, 5 classes) and a long-tail dataset of gastro-intestinal video frames (10K images, 23 classes), using two CNNs of varying representation capabilities. Experimental results demonstrate that applying Balanced-MixUp outperforms other conventional sampling schemes and loss functions specifically designed to deal with imbalanced data. Code to reproduce our results is released at \url{github.com/...}.


==> table_0.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.0}	
\centering
\setlength\tabcolsep{6pt}
\caption{Definition of the Closed/Open Set partitions on the two considered datasets. In the Kather-5K there are eight categories, whereas in the Kather-100k there are nine, see the text for acronym definitions and motivation.}
\label{os_splits}
\begin{tabular}{l cc}
\midrule
                   & \multicolumn{1}{c}{Kather-5K Closed Set $\mathcal{C}^{5k}_i$} & \multicolumn{1}{c}{Kather-100K Closed Set $\mathcal{C}^{100k}_i$}  \\
    \cmidrule(lr){2-2} \cmidrule(lr){3-3} 
Split $\mathcal{S}_1$               & \makecell{TUM, SIM-STR, COM-STR, \\LYM, NORM}   &  \makecell{TUM, TUM-STR, \\MUSC, LYM, NORM} \\
\midrule
Split $\mathcal{S}_2$               & TUM, SIM-STR, COM-STR        &  TUM, TUM-STR \\
\midrule
Split $\mathcal{S}_3$               & TUM, SIM-STR, COM-STR, LYM             &  TUM, TUM-STR, MUS                        \\
\bottomrule
\end{tabular}
\end{table}

